Managing Bandwidth: The Key to Cloud-Assisted Autonomous Driving

Prevailing wisdom asserts that one cannot rely on the cloud for critical real-time control systems like self-driving cars. We argue that we can, and must. Following the trends of increasing model sizes, improvements in hardware, and evolving mobile networks, we identify an opportunity to offload parts of time-sensitive and latency-critical compute to the cloud. Doing so requires carefully allocating bandwidth to meet strict latency SLOs, while maximizing benefit to the car.

==> Makefile <==
LATEX := pdflatex

all: paper.pdf

BIB := $(shell find . -name '*.bib')
FIGS := $(shell find figures/ -name '*.pdf')
TIKZ := $(shell find figures/ -name '*.tikz')
TEX := $(shell find . -name '*.tex')
EXTS = *.aux *.backup *.blg *.log *.out *.lof *.loa *.lot *.toc *.bbl *.bak \
       *.texshop *.dvi *.fdb_latexmk *.fls *.ent *.run.xml *.run.xml

paper.pdf: ${TEX}  ${TIKZ} ${BIB} ${FIGS}
	latexmk -pdf -bibtex paper.tex

push:
	scp paper.pdf pschafhalter@como:public_html/pub/drafts/2024-tradeoffs-av-remote-resources-hotnets.pdf

clean:
	latexmk -C
	rm -f paper.pdf
	rm -f ${EXTS}

